Rio: A System Solution for Sharing I/O between Mobile Systems

Mobile systems are equipped with a diverse collection of I/O devices, including cameras, microphones, sensors, and modems. There exist many novel use cases for allowing an application on one mobile system to utilize I/O devices from another. This paper presents Rio, an I/O sharing solution that supports unmodified applications and exposes all the functionality of an I/O device for sharing. Rio's design is common to many classes of I/O devices, thus significantly reducing the engineering effort to support new I/O devices. Our implementation of Rio on Android consists of 6700 total lines of code and supports four I/O classes with fewer than 450 class-specific lines of code. Rio also supports I/O sharing between mobile systems of different form factors, including smartphones and tablets. We show that Rio achieves performance close to that of local I/O for audio, sensors, and modems, but suffers noticeable performance degradation for camera due to network throughput limitations between the two systems, which is likely to be alleviated by emerging wireless standards.

==> discussions.tex <==
\section{Limitations and Future Work}

The current design of Rio has limitations. Below we introduce these
limitations and explain our plans to overcome some of them in our future
work.

\subsection{Supporting other I/O devices}

There are several other classes of I/O devices that we plan to support
in our future work. This includes the GPU (for graphics and
computation), touchscreen, GPS, and FM radio.
%Supporting high performance GPU graphics would be challenging with no
%further optimizations as the GPU HAL and driver use many file operations
%per frame. Techniques are required to parallelize these file operations
%without modifications to the HAL nor the driver so that the file
%operations can be batched in Rio.

There are, however, two classes of I/O that Rio's design cannot support
including network and block devices. This is because these I/O
devices do not use the device file interface for communications between
the process and the driver. Network devices use sockets along with the kernel
networking stack and block devices use file systems.

\subsection{I/O Sharing with Untrusted Systems}
\label{sec:discussions_untrusted}

In this paper, we assumed that the systems sharing I/O through Rio trust
each other not to be malicious (\S\ref{sec:design_guarantees}).
Supporting untrusted systems creates new challenges for Rio, which fall into two
categories.

{\bf Protecting the server:} As also discussed
in~\cite{AmiriSani2014}, device drivers are buggy and malicious
applications can abuse these bugs through the device file interface to
compromise the driver protection domain~\cite{BUG1, BUG2}. In Rio, this
means that a malicious process in the client can compromise the server,
e.g., through privilege escalation. In order to solve this problem, the
device driver and the device need to be sandboxed in a protection
domain in the server, using techniques similar to~\cite{AmiriSani2014}, 
%. Techniques similar to
Nooks~\cite{Swift2003}, and VirtuOS~\cite{Nikolaev2013}.
% can be used for
%the sandbox inside the server.

{\bf Protecting the client:} An untrusted
server can issue spurious copy memory operations to the client in order
to compromise the client.  The client stub can simply protect against
this threat by strictly checking the copy memory operations requested by
the server, similar to~\cite{AmiriSani2014}.

Note that the server can also snoop
the client's data that are shared with the I/O device in the server,
e.g., the audio segments.
%it can store the audio segments that the client plays through the
%server's speaker. 
Since the server is completely untrusted, we cannot
provide any isolation for the client's data. This is indeed an inherent
problem to any I/O sharing systems, and not specific to Rio.

\subsection{Supporting other OSes}

iOs, the other major mobile system, also uses device files and hence can
be supported in Rio. Sharing I/O devices between iOS systems should
require similar engineering effort reported in this paper for sharing
I/O devices between Android systems.  However, sharing I/O devices
between iOS an Android require potentially more and non-trivial
engineering effort, mainly because these two OSes have different I/O
stack designs and hence different I/O device API.

%\note{I/O Power Management?}

